The Third Monocular Depth Estimation Challenge

This paper discusses the results of the third edition of the Monocular Depth Estimation Challenge (MDEC). The challenge focuses on zero-shot generalization to the challenging SYNS-Patches dataset, featuring complex scenes in natural and indoor settings. As with the previous edition, methods can use any form of supervision, i.e. supervised or self-supervised. The challenge received a total of 19 submissions outperforming the baseline on the test set: 10 among them submitted a report describing their approach, highlighting a diffused use of foundational models such as Depth Anything at the core of their method. The challenge winners drastically improved 3D F-Score performance, from 17.51% to 23.72%.

==> Figures/depth.tex <==
% SYNS-Patches Depth Visualizations

\tiny

\def\first{0639}
\def\nums{0389,0039,0621,0682,0599,0745,0763}
\def\dataset{SynsDepth}

% \def\second{0556}
% \def\numss{0226,0044,0051,0656,0462,0739,0747}
% \def\datasett{SynsDepth2}


\def\methods{
    img/
    ,gt/GT
    ,zhouguangyuan/PICO-MR
    ,jsk24/RGA-Robot
    ,lavreniuk/EVP++
    ,Depth\_3DV/3DCreators
    ,surajiitd/visioniitd
    ,pihai/HIT-AIIA
    ,weijianing/FRDC-SH
    ,hyc123/hyc123
    ,al/ReadingLS
    ,mdec/Baseline   
    %,dagouqin/dagouqin
    %,erdosv001/erdosv001
    %,hitcslj/hitcslj
    %,inso/inso
    %,journey2japan/journey2japan    
    %,luo0207/luo0207
    %,moyushin/moyushin    
    %,qing/qing
    %,SmartHust/SmartHust
    ,smhh/Elder Lab    
    %,yogurts/yogurts
}

    % ,mdec/\team{0}
    % ,al/\team{0}
    % ,dagouqin/\team{0}
    % ,Depth_3DV/\team{0}
    % ,erdosv001/\team{0}
    % ,hitcslj/\team{0}
    % ,hyc123/\team{0}
    % ,inso/\team{0}
    % ,journey2japan/\team{0}
    % ,jsk24/\team{0}
    % ,lavreniuk/\team{0}
    % ,luo0207/\team{0}
    % ,moyushin/\team{0}
    % ,pihai/\team{0}
    % ,qing/\team{0}
    % ,SmartHust/\team{0}
    % ,smhh/\team{0}
    % ,surajiitd/\team{0}
    % ,weijianing/\team{0}
    % ,yogurts/\team{0}
    % ,zhouguangyuan/\team{0}

\def\w{0.12\linewidth}

\foreach \method/\label in \methods{%
    \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0,anchor=south west}]
        \node (image) at (0, 0) {\includegraphics[width=\w]{\dataset/\first_\method.jpg}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw (0.01, 0.01) node {\color{white}{\textbf{\label}}};
        \end{scope}
    \end{tikzpicture}
    %
    \foreach \num in \nums{%
        \includegraphics[width=\w]{\dataset/\num_\method.jpg}
    } \\
}

% \vspace{1em}

% \foreach \method/\label in \methods{%
%     \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0,anchor=south west}]
%         \node (image) at (0, 0) {\includegraphics[width=\w]{\datasett/\second_\method.jpeg}};
%         \begin{scope}[x={(image.south east)},y={(image.north west)}]
%             \draw (0.01, 0.01) node {\color{white}{\textbf{\label}}};
%         \end{scope}
%     \end{tikzpicture}
%     %
%     \foreach \num in \numss{%
%         \includegraphics[width=\w]{\datasett/\num_\method.jpeg}
%     } \\
% }

%\todo{Update images and participants}

\mycaption{\acl{syns} Depth Visualization}{%
Best viewed in color and zoomed in. Methods are ranked based on their F-Score in \tbl{res:results}. 
We can appreciate how thin structures still represent one of the hardest challenges to any method, such as branches and railings, for instance. 
Near depth discontinuities, most approaches tend to produce ``halos'', interpolating between foreground and background objects and thus failing to perceive sharp boundaries.
%caused by interpolation between foreground and background objects. 
%Notable improvements can be seen in Natural and Agricultural scenes, where the top submissions provide much higher levels of detail than the baseline. 
Nonetheless, most methods expose higher level of detail compared to the baseline.
}


==> Figures/distrib.tex <==
% SYNS-Patches Depth Distribution

\includegraphics[width=0.8\textwidth]{Images/syns_scenes_stats.png} \\
\includegraphics[width=1\linewidth]{Images/depth_distrib.pdf}\\\vspace{-0.3cm}
\mycaption{\acl{syns} Properties}{%
%Indoor scenes are limited to 20m, while outdoor scenes reach up to 120m. 
Top: Distribution of images per category in the validation split and the test split respectively. Bottom: Depth distribution per scene type -- indoor scenes are limited to 20m, while outdoor scenes reach up to 120m; natural and Agriculture scenes contain a larger percentage of long-range depths (20-80m), while urban scenes focus on the mid-range (20-40m).
% \mycaption{Depth Distribution Per Scene Type}{%
% Indoor scenes are limited to 20m, while outdoor scenes reach up to 120m. 
% Natural and Agriculture scenes contain a larger percentage of long-range depths (20-80m), while urban scenes focus on the mid-range (20-40m).
}


==> Figures/syns.tex <==
% SYNS-Patches Sample Images

% \foreach \img in {img, gt, edge}{%
%     \foreach \num in {0064, 0131, 0156, 0183}{%
%         \includegraphics[width=0.25\linewidth]{Syns/\num_\img.jpeg}%
%     }\\\vspace{-1pt}%
% }
% \vspace{0.1cm}
% \foreach \img in {img, gt, edge}{%
%     \foreach \num in {0234, 0337, 0352, 0367}{%
%         \includegraphics[width=0.25\linewidth]{Syns/\num_\img.jpeg}%
%     }\\\vspace{-1pt}%
% }

% \foreach \img in {img, gt, edge}{%
%     \foreach \num in {0012, 0042, 0090, 0120}{%
%         \includegraphics[width=0.25\linewidth]{Syns_2024/\num_\img.jpeg}%
%     }\\\vspace{-1pt}%
% }
% \vspace{0.1cm}
% \foreach \img in {img, gt, edge}{%
%     \foreach \num in {0350, 0450, 0712, 0730}{%
%         \includegraphics[width=0.25\linewidth]{Syns_2024/\num_\img.jpeg}%
%     }\\\vspace{-1pt}%
% }

\foreach \img in {img, gt, edge}{%
    \foreach \num in {0012, 0450, 0120, 0730}{%
        \includegraphics[width=0.25\linewidth]{Syns_2024/\num_\img.jpeg}%
    }\\\vspace{-1pt}%
}
% \vspace{0.1cm}
% \foreach \img in {img, gt, edge}{%
%     \foreach \num in {0350, 0450, 0712, 0730}{%
%         \includegraphics[width=0.25\linewidth]{Syns_2024/\num_\img.jpeg}%
%     }\\\vspace{-1pt}%
% }

\mycaption{\acl{syns} Dataset}{%
We show samples from diverse scenes, including complex urban, natural, and indoor spaces. 
%The dataset contains 
High-quality ground-truth depth covers about 78.20\% of the image, from which depth boundaries are computed as Canny edges in log space.
}


==> Tables/datasets.tex <==
% Dataset Statistics

\mycaption{Dataset \& Benchmark Comparison}{%
We summarize recent datasets commonly used in self-supervised monocular depth estimation. 
CityScapes represents a common pretraining dataset, while \acl{syns} is testing-only.
\acl{syns} is the only dataset providing high-quality dense depth maps in a wide variety of environments.
}

\begin{tabular}{llllllllll}
\toprule
                                                  &    Accuracy & Density (\%) &  Num Points &  Urban & Natural &  Indoor &   Train &     Val &    Test \\
\midrule
                     CityScapes~\cite{Cordts2016} &      \xmark &       \xmark &      \xmark & \cmark &  \xmark &  \xmark &  88,250 &  \xmark &  \xmark \\
      Kitti Eigen-Zhou~\cite{Geiger2013,Zhou2017} &      \xmark &       \xmark &      \xmark & \cmark &  \xmark &  \xmark &  39,810 &   4,424 &  \xmark \\
\midrule
          Kitti Eigen~\cite{Geiger2013,Eigen2015} &         Mid &         4.10 &         19k & \cmark &  \xmark &  \xmark &  45,200 &   1,776 &     697 \\
Kitti Eigen-Benchmark~\cite{Geiger2013,Uhrig2018} &        High &        15.28 &         71k & \cmark &  \xmark &  \xmark &  71,633 &   5,915 &     652 \\
                        DDAD~\cite{Guizilini2020} &        High &         1.02 &         24k & \cmark &  \xmark &  \xmark &  75,900 &  23,700 &   3,080 \\
\midrule
          \acl{syns}~\cite{Adams2016,Spencer2022} &        High &        78.30 &        365k & \cmark &  \cmark &  \cmark &  \xmark &     400 &     775 \\
\bottomrule
\end{tabular}


==> Tables/results.tex <==
% SYNS-Patches Results

\footnotesize

\def\n{9}

\mycaption{\acl{syns} Results}{%
%We provide metrics across the whole dataset and per scene-category. 
%As expected, supervised methods generally outperform self-supervised ones. 
%The largest gap can be found in Indoor scenes, self-supervised methods were trained exclusively on automotive data. 
%Teams~\team{4} \& \team{5} outperformed the challenge baseline~\cite{Spencer2022} by incorporating more advanced network architectures.
We provide metrics across the whole test split of the dataset. Top-performing entries generally leverage the pre-trained Depth Anything \cite{Yang2024} model. Only a few methods use self-supervised losses or proxy depth labels.
}\vspace{-0.3cm}

\begin{tabular}{@{}rrrrrrrrrrr@{}}
\toprule
                                           &            & Train & Rank &        F\up & F-Edges\up &     MAE\down &    RMSE\down &      AbsRel\down & Acc-Edges\down & Comp-Edges\down \\ 
\midrule           
            
           &  \team{1} & \train{1} &  \best{1} & \best{23.72} & \nbest{11.01} & \nbest{3.78} & \nbest{6.61} & 21.24 & 3.90 & 4.45 \\ 
           &  \team{2} & \train{2} & \nbest{2} & \nbest{23.25} & 10.78 & 3.87 & 6.70 & 21.70 & 3.59 & 9.86 \\ 
           &  \team{3} & \train{3} &         3 & 22.79 & \best{11.52} & 5.21 & 9.23 & 28.86 & 4.15 & \nbest{0.90} \\ 
           &  \team{4} & \train{4} &         4 & 20.87 & 10.92 & \best{3.71} & \best{6.53} & \best{19.02} & 2.88 & 6.77 \\ 
           &  \team{5} & \train{5} &         5 & 20.77 & 9.96 & 4.33 & 7.83 & 27.80 & 3.45 & 13.25 \\ 
           &  \team{6} & \train{6} &         6 & 20.42 & 10.19 &	4.41 &	7.89 &	23.94 &	3.61 &	5.80 \\ 
           & \team{7} & \train{7} &           7 & 19.07 & 9.92 & 4.53 & 7.96 & 23.27 & 3.26 & 8.00 \\
           &  \team{8} & \train{8} &         8 & 18.60 &	9.43 &	3.92 &	7.16 &	\nbest{20.12} &	2.89 &	15.65 \\ 
           &  \team{9} & \train{9} &        9 & 17.83 &	9.14 &	4.11 &	7.73 &	21.23 &	2.95 &	17.81 \\
           &  \team{10} & \train{10} &        10 & 17.81 &	9.75 &	5.04 &	8.92 &	24.01 &	3.16 &	14.16 \\
           &  \team{11} & \train{11} &        11 & 17.57 &	9.13 &	4.28 &	8.36 &	23.35 &	3.18 &	20.66 \\
           &  \team{12} & \train{12} &        12 & 16.91 &	9.07 &	4.14 &	7.35 &	22.05 &	3.24 &	18.52 \\
           &  \team{13} & \train{13} &        13 & 16.71 &	9.25 &	5.48 &	11.05 &	34.20 &	\best{2.57} &	18.04 \\
           &  \team{14} & \train{14} &        14 & 16.45 &	8.89 &	5.29 &	10.53 &	33.67 &	\nbest{2.60} &	18.73 \\
           &  \team{15} & \train{15} &        15 & 15.92 &	9.17 &	8.25 &	13.88 &	43.88 &	4.11 &	\best{0.74} \\
           &  \team{16} & \train{16} &        16 & 14.81 &	8.14 &	5.01 &	8.94 &	29.39 &	3.28 &	30.28 \\
           &  \team{0} & \train{0} &        17 & 13.72 &	7.76 &	5.56 &	9.72 &	32.04 &	3.97 &	21.63 \\
           &  \team{17} & \train{17} &        18 & 13.71 &	7.55 &	5.49 &	9.44 &	30.74 &	3.61 &	18.36 \\
           &  \team{18} & \train{18} &        19 & 11.90 &	8.08 &	6.33 &	10.89 &	30.46 &	2.99 &	33.63 \\
           &  \team{19} & \train{19} &        20 & 11.04 & 7.09 & 8.76 & 15.86 & 63.32 & 3.22 & 40.61 \\

           % &  \team{1} & \train{1} &  \best{1} & 23.7210 & 11.0130 & 3.7787 & 6.6115 & 21.2386 & 3.8974 & 4.4517 \\ 
           % &  \team{2} & \train{3} & \nbest{2} & 23.2499 & 10.7783 & 3.8725 & 6.7038 & 21.6987 & 3.5911 & 9.8569 \\ 
           % &  \team{3} & \train{3} &         3 & 22.7924 & 11.5192 & 5.2061 & 9.2339 & 28.8613 & 4.1541 & 0.8980 \\ 
           % &  \team{4} & \train{5} &         4 & 20.8658 & 10.9224 & 3.7086 & 6.5308 & 19.0214 & 2.8835 & 6.7700 \\ 
           % &  \team{5} & \train{6} &         5 & 20.7673 & 9.9617 & 4.3302 & 7.8348 & 27.7973 & 3.4458 & 13.2527 \\ 
           % &  \team{6} & \train{8} &         6 & 20.4244 & 10.1868 &	4.4079 &	7.8909 &	23.9416 &	3.6105 &	5.7953 \\ 
           % &  \team{7} & \train{4} &         7 & 18.5956 &	9.4273 &	3.9224 &	7.1649 &	20.1185 &	2.8921 &	15.6460 \\ 
           % &  \team{8} & \train{7} &         8 & 18.4475 &	9.7061 &	4.7358 &	8.6001 &	25.6061 &	3.3700 &	6.6398 \\
           % &  \team{10} & \train{8} &        10 & 17.8328 &	9.1387 &	4.1147 &	7.7332 &	21.2310 &	2.9465 &	17.8145 \\
           % &  \team{11} & \train{8} &        11 & 17.8121 &	9.7525 &	5.0386 &	8.9196 &	24.0101 &	3.1615 &	14.1550 \\
           % &  \team{12} & \train{8} &        12 & 17.5704 &	9.1273 &	4.2759 &	8.3635 &	23.3455 &	3.1765 &	20.6621 \\
           % &  \team{13} & \train{8} &        13 & 16.9120 &	9.0666 &	4.1357 &	7.3481 &	22.0509 &	3.2377 &	18.5220 \\
           % &  \team{14} & \train{8} &        14 & 16.7148 &	9.2525 &	5.4767 &	11.0510 &	34.2035 &	2.5703 &	18.0436 \\
           % &  \team{15} & \train{8} &        15 & 16.4478 &	8.8896 &	5.2907 &	10.5310 &	33.6741 &	2.5965 &	18.7283 \\
           % &  \team{16} & \train{8} &        16 & 15.9223 &	9.1679 &	8.2542 &	13.8783 &	43.8823 &	4.1054 &	0.7403 \\
           % &  \team{17} & \train{8} &        17 & 14.8093 &	8.1357 &	5.0099 &	8.9448 &	29.3938 &	3.2837 &	30.2778 \\
           % &  \team{0} & \train{0} &        18 & 13.7211 &	7.7630 &	5.5645 &	9.7169 &	32.0420 &	3.9712 &	21.6256 \\
           % &  \team{18} & \train{8} &        19 & 13.7089 &	7.5505 &	5.4867 &	9.4419 &	30.7377 &	3.6072 &	18.3600 \\
           % &  \team{19} & \train{8} &        20 & 11.8998 &	8.0770 &	6.3256 &	10.8861 &	30.4607 &	2.9862 &	33.6279 \\
           %&  \team{20} & \train{8} &        21 & 11.0444 & 7.0866 & 8.7645 & 15.8637 & 63.3160 & 3.2209 & 40.6098 \\
\bottomrule
\end{tabular}

\emph{
\textbf{M}=Monocular -- \textbf{S}=Stereo -- \textbf{D*}=Proxy Depth -- \textbf{D}=Ground-truth Depth -- \textbf{$\dagger$}=Pre-trained Depth Anything model
}


==> Tables/results_2023.tex <==
% SYNS-Patches Results

\footnotesize

\def\n{9}

\mycaption{\acl{syns} Results}{%
We provide metrics across the whole dataset and per scene-category. 
As expected, supervised methods generally outperform self-supervised ones. 
The largest gap can be found in Indoor scenes, self-supervised methods were trained exclusively on automotive data. 
Teams~\team{4} \& \team{5} outperformed the challenge baseline~\cite{Spencer2022} by incorporating more advanced network architectures.
}

\begin{tabular}{@{}lllllllllll@{}}
\toprule
                                           &            & Train & Rank &        F\up & F-Edges\up &     MAE\down &    RMSE\down &      AbsRel\down & Acc-Edges\down & Comp-Edges\down \\ 
\midrule           
            
            \multirow{\n}*{\emph{Overall}} &  \team{1} & \train{1} &  \best{1} &  \best{17.51} &         8.80 &  \best{4.52} &         8.72 &  \best{24.32} &         3.22 &         21.65 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} & \nbest{16.94} &  \best{9.63} & \nbest{4.71} &  \best{8.00} &         25.35 &         3.56 &         19.95 \\ 
                                           &  \team{3} & \train{3} &         3 &         16.70 & \nbest{9.36} &         4.91 &         8.63 & \nbest{24.33} &  \best{3.02} &         18.07 \\ 
                                           &  \team{5} & \train{5} &         4 &         16.00 &         8.49 &         5.08 &         8.96 &         28.46 &         3.74 &  \best{11.32} \\ 
                                           &  \team{6} & \train{6} &         5 &         14.71 &         8.13 &         5.17 &         8.97 &         29.43 &         3.75 & \nbest{17.29} \\ 
                                           &  \team{0} & \train{0} &         6 &         13.72 &         7.76 &         5.56 &         9.72 &         32.04 &         3.97 &         21.63 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         13.23 &         8.26 &         5.18 &         8.76 &         28.03 & \nbest{3.07} &         29.96 \\ 
                                           &  \team{4} & \train{4} &         7 &         12.77 &         7.68 &         5.17 &         8.83 &         29.92 &         3.56 &         35.26 \\ 
                                           &  \team{7} & \train{7} &         8 &         12.44 &         7.49 &         5.05 & \nbest{8.59} &         28.99 & \nbest{3.10} &         38.93 \\ 
                                           &  \team{8} & \train{8} &        9 &         11.29 &         7.18 &         5.81 &         9.58 &         32.82 &         3.47 &         43.38 \\ 
                                        %   &\team{10} & \train{10} &        11 &          9.99 &         6.74 &         5.95 &         9.69 &         34.49 &         3.51 &         47.95 \\ 
\midrule
      \multirow{\n}*{\emph{Outdoor-Urban}} &  \team{1} & \train{1} &  \best{1} &  \best{16.41} &         7.37 &  \best{3.81} &         7.82 &  \best{21.85} &         2.91 &         24.36 \\ 
                                           &  \team{5} & \train{5} &         4 & \nbest{16.28} &         7.27 &         4.49 &         7.98 &         26.18 &         3.67 &  \best{13.11} \\ 
                                           &  \team{6} & \train{6} &         5 &         15.21 &         6.80 &         4.60 &         8.00 &         27.55 &         3.73 &         16.26 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} &         15.10 &  \best{8.48} & \nbest{4.03} &  \best{6.90} &         23.67 &         3.36 &         19.13 \\ 
                                           &  \team{3} & \train{3} &         3 &         15.01 & \nbest{7.79} &         4.26 &         7.70 & \nbest{22.88} & \nbest{2.87} & \nbest{15.73} \\ 
                                           &  \team{0} & \train{0} &         6 &         14.09 &         6.48 &         4.77 &         8.43 &         29.10 &         3.89 &         22.75 \\ 
                                           &  \team{4} & \train{4} &         7 &         12.90 &         5.92 &         4.49 &         7.80 &         27.44 &         3.26 &         35.36 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         12.53 &         6.43 &         4.61 &         7.93 &         26.28 &  \best{2.82} &         27.07 \\ 
                                           &  \team{7} & \train{7} &         8 &         12.52 &         5.89 &         4.37 & \nbest{7.62} &         26.46 &  \best{2.83} &         40.33 \\ 
                                           &  \team{8} & \train{8} &         9 &         11.31 &         5.73 &         5.14 &         8.69 &         30.64 &         3.13 &         40.15 \\ 
                                        %   &\team{10} & \train{10} &        11 &          9.95 &         5.18 &         5.20 &         8.73 &         32.12 &         3.15 &         43.54 \\ 
\midrule   
    \multirow{\n}*{\emph{Outdoor-Natural}} &  \team{2} & \train{3} & \nbest{2} &  \best{14.90} & \nbest{6.75} & \nbest{6.26} &  \best{10.47} &         28.40 &         3.54 &         14.44 \\ 
                                           &  \team{3} & \train{3} &         3 & \nbest{14.66} &  \best{6.79} &         6.35 &         10.86 & \nbest{27.09} &  \best{3.08} &         19.73 \\ 
                                           &  \team{5} & \train{5} &         4 &         14.43 &         6.02 &         6.51 &         11.43 &         30.57 &         3.59 &   \best{9.44} \\ 
                                           &  \team{1} & \train{1} &  \best{1} &         14.31 &         6.07 &  \best{5.97} & \nbest{10.81} &  \best{26.48} &         3.45 &         17.75 \\ 
                                           &  \team{6} & \train{6} &         5 &         12.89 &         5.74 &         6.77 &         11.62 &         32.57 &         3.68 & \nbest{13.97} \\ 
                                           &  \team{0} & \train{0} &         6 &         12.10 &         5.32 &         7.46 &         12.86 &         36.89 &         3.84 &         18.35 \\ 
                                           &  \team{4} & \train{4} &         7 &         11.54 &         6.03 &         6.87 &         11.52 &         33.66 &         3.36 &         32.47 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         11.28 &         6.12 &         6.75 &         11.02 &         32.03 & \nbest{3.09} &         28.65 \\ 
                                           &  \team{7} & \train{7} &         8 &         10.98 &         5.38 &         6.66 &         11.13 &         32.19 & \nbest{3.13} &         36.01 \\ 
                                           &  \team{8} & \train{8} &         9 &          9.26 &         4.92 &         7.69 &         12.22 &         38.14 &         3.36 &         42.92 \\ 
                                        %   &\team{10} & \train{10} &        11 &          7.73 &         4.33 &         7.91 &         12.41 &         40.51 &         3.39 &         47.33 \\ 
\midrule   
\multirow{\n}*{\emph{Outdoor-Agriculture}} &  \team{1} & \train{1} &  \best{1} &  \best{16.36} &         5.24 &  \best{5.17} &        10.13 &         29.07 &         3.43 &         18.84 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} & \nbest{15.58} &  \best{6.40} & \nbest{5.25} &  \best{9.09} & \nbest{27.45} &         3.64 &         18.30 \\ 
                                           &  \team{5} & \train{5} &         4 &         14.94 &         5.49 &         5.70 &        10.14 &         30.70 &         3.75 &  \best{10.27} \\ 
                                           &  \team{3} & \train{3} &         3 &         14.68 & \nbest{5.82} &         5.61 &        10.02 &  \best{25.90} &  \best{3.17} &         17.67 \\ 
                                           &  \team{6} & \train{6} &         5 &         14.03 &         5.06 &         5.65 &         9.98 &         30.40 &         3.80 & \nbest{15.94} \\ 
                                        %   &  \team{9} & \train{9} &         7 &         12.67 &         4.92 &         5.76 &        10.04 &         29.48 &         3.18 &         29.39 \\ 
                                           &  \team{0} & \train{0} &         6 &         12.26 &         4.76 &         6.10 &        10.84 &         33.58 &         4.00 &         18.73 \\ 
                                           &  \team{4} & \train{4} &         7 &         11.56 &         4.55 &         5.61 &         9.79 &         31.16 &         3.60 &         35.30 \\ 
                                           &  \team{7} & \train{7} &         8 &         11.15 &         4.52 &         5.62 & \nbest{9.61} &         31.43 & \nbest{3.17} &         39.06 \\ 
                                           &  \team{8} & \train{8} &         9 &         10.27 &         3.97 &         6.34 &        10.76 &         33.61 &         3.40 &         38.73 \\ 
                                        %   &\team{10} & \train{10} &        11 &          8.42 &         3.41 &         6.52 &        10.91 &         35.61 &         3.42 &         43.22 \\ 
\midrule   
            \multirow{\n}*{\emph{Indoor}}  &  \team{1} & \train{1} &  \best{1} &  \best{33.20} & \nbest{33.12} &  \best{0.70} &         1.63 &  \best{13.08} &  \best{2.89} &         33.52 \\ 
                                           &  \team{3} & \train{3} &         3 & \nbest{33.08} &  \best{33.57} &         0.87 & \nbest{1.35} &         16.52 & \nbest{2.90} & \nbest{21.76} \\ 
                                           &  \team{2} & \train{3} & \nbest{2} &         32.05 &         32.53 & \nbest{0.83} &  \best{1.26} & \nbest{16.00} &         4.11 &         45.68 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         22.55 &         31.29 &         0.85 & \nbest{1.27} &         17.90 &         3.49 &         45.80 \\ 
                                           &  \team{5} & \train{5} &         4 &         22.49 &         29.53 &         1.06 &         1.59 &         23.38 &         4.38 &  \best{14.52} \\ 
                                           &  \team{0} & \train{0} &         6 &         21.11 &         28.96 &         1.04 &         1.51 &         22.77 &         4.60 &         37.09 \\ 
                                        %   & \team{10} & \train{10} &        11 &         20.84 &         29.76 &         1.03 &         1.49 &         21.12 &         5.40 &         78.85 \\ 
                                           &  \team{6} & \train{6} &         5 &         20.25 &         29.52 &         1.03 &         1.48 &         23.37 &         3.96 &         35.68 \\ 
                                           &  \team{7} & \train{7} &         8 &         19.82 &         28.62 &         0.97 &         1.42 &         20.91 &         3.63 &         43.46 \\ 
                                           &  \team{8} & \train{8} &         9 &         19.81 &         28.93 &         1.02 &         1.49 &         21.83 &         5.19 &         69.50 \\ 
                                           &  \team{4} & \train{4} &         7 &         19.18 &         28.34 &         1.09 &         1.61 &         23.24 &         5.14 &         44.02 \\ 
\bottomrule
\end{tabular}

\emph{
\textbf{M}=Monocular -- \textbf{S}=Stereo -- \textbf{D*}=Proxy Depth -- \textbf{D}=Ground-truth Depth
}


==> Tables/syns_cat.tex <==

% SYNS-Patches Category Distribution

% \mycaption{\acl{syns}}{Distribution of images per category in the val/test splits.}

% \begin{tabular}{@{}llllllllll|l@{}}
% \toprule
%                & Agriculture & Indoor & Industry & Misc & Natural & Recreation & Residential & Transport & Woodland & Total \\ 
% \midrule
%   \textbf{Val} &         104 &     67 &       36 &   72 &      36 &         14 &          13 &         4 &       54 &   400 \\ 

%  \textbf{Test} &         211 &     81 &       71 &    0 &     147 &         48 &         110 &        17 &       90 &   775 \\ 
% \midrule
% \textbf{Total} &         315 &    148 &      107 &   72 &     183 &         62 &         123 &        21 &      144 & 1,175 \\ 
% \bottomrule
% \end{tabular}

